Lexico: Extreme KV Cache Compression via Sparse Coding over Universal Dictionaries

We introduce Lexico, a novel KV cache compression method that leverages sparse coding with a universal dictionary. Our key finding is that key-value cache in modern LLMs can be accurately approximated using sparse linear combination from a small, input-agnostic dictionary of ~4k atoms, enabling efficient compression across different input prompts, tasks and models. Using orthogonal matching pursuit for sparse approximation, Lexico achieves flexible compression ratios through direct sparsity control. On GSM8K, across multiple model families (Mistral, Llama 3, Qwen2.5), Lexico maintains 90-95% of the original performance while using only 15-25% of the full KV-cache memory, outperforming both quantization and token eviction methods. Notably, Lexico remains effective in low memory regimes where 2-bit quantization fails, achieving up to 1.7x better compression on LongBench and GSM8K while maintaining high accuracy.

==> section/background.tex <==
\section{Background}

\subsection{Preliminary and Notations}

Most pre-trained \glspl{llm} utilize a decoder-only transformer architecture. Within each layer of the transformer, multi-head self-attention with a causal mask is applied. Let the input token embeddings be denoted as $\mX \in \sR^{l_{\text{seq}} \times d}$, where $l_{\text{seq}}$ represents the sequence length. For simplicity, we focus on a single layer and express the output computation for each attention head $\mH^{(h)}$ as:
\begin{equation} 
    \mH^{(h)} = \text{Softmax} \left( \text{Mask} \left( \frac{\mQ^{(h)} \mK^{(h)\top}}{\sqrt{m}} \right) \right) \mV^{(h)}, 
\end{equation}
where the query, key, and value matrices are linear projections of the input token embeddings: $\mQ^{(h)} = \mX \mW_q^{(h)}, \quad \mK^{(h)} = \mX \mW_k^{(h)}, \quad \mV^{(h)} = \mX \mW_v^{(h)}$, with $\mW_q^{(h)}, \mW_k^{(h)}, \mW_v^{(h)} \in \mathbb{R}^{d \times m}$ being the model weights and $m$ representing the head dimension.

In the context of causal attention, the key ($\mK$) and value ($\mV$) states for preceding tokens do not depend on subsequent tokens. Therefore, during autoregressive decoding, the $\mK$ and $\mV$ states are cached to prevent recomputation, thereby speeding up the decoding process.

Let $t$ represent the current step in the autoregressive decoding, and let $\vx_t \in \mathbb{R}^{1 \times d}$ denote the embedding of the newly generated token. The key and value caches, up to but not including the current token, are denoted as $\mK_{t-1}^{(h)}$ and $\mV_{t-1}^{(h)}$, respectively. The typical autoregressive decoding process using the \gls{kv} cache can be expressed as:
\begin{equation} \label{eq:attention_with_kv_cache}
    \vh_t^{(h)} = \text{Softmax} \left( \frac{\vq_t^{(h)} \left( \mK_{t-1}^{(h)} \parallel \vk_t^{(h)} \right)^\top}{\sqrt{m}} \right) \left( \mV_{t-1}^{(h)} \parallel \vv_t^{(h)} \right), 
\end{equation}
where $\vq_t^{(h)}, \vk_t^{(h)}, \vv_t^{(h)}$ represent the query, key, and value vectors for the new token embedding $\vx_t$. Here, $\parallel$ denotes concatenation along the sequence length dimension.

\subsection{Dictionary-based Data Compression via Sparse Representation}

Sparse representation has proven to be a powerful technique for information compression across various domains, including image compression, signal processing, and medical imaging. In sparse representation, a signal $\vk \in \mathbb{R}^m$ is approximated as a linear combination of a limited number of basis elements, commonly referred to as atoms, from an overcomplete dictionary $\mD \in \mathbb{R}^{m \times n}$. This reconstruction is given by the expression:
\begin{equation}
    \vk = \mD \vy,
\end{equation}
where $\vy$ is the sparse representation vector that encodes the linear combination of the atoms. The sparsity of this representation is defined by $s = || \vy ||_0$, representing the number of non-zero elements in $\vy$. While $m < n$, storing the signal via $\vy \in \mathbb{R}^n$ rather than $\vk \in \mathbb{R}^m$ can be beneficial, as specialized algorithms and data structures can be employed to leverage the sparsity of $\vy$.

The problem of determining the optimal sparse representation—minimizing the sparsity while ensuring a small reconstruction error—is NP-hard. This optimization problem is typically formulated as:
\begin{equation}
    \underset{\vy}{\text{min}} \left\| \vy \right\|_0 \quad \text{subject to} \quad \frac{\left\| \vk - \mD \vy \right\|_2}{\left\| \vk \right\|_2} \leq \delta \quad \text{for some} \quad \delta \geq 0
\end{equation}

Algorithms designed to solve this minimization problem are referred to as sparse approximation algorithms.
